Optimized Soft-Aided Decoding of OFEC and Staircase Codes

We propose a novel soft-aided hard-decision decoding algorithm for general product-like codes. It achieves error correcting performance similar to that of a soft-decision turbo decoder for staircase and OFEC codes, while maintaining a low complexity.

==> plots/stall_pattern.tex <==
\begin{tikzpicture}
    \begin{axis}[
        compat=newest,
        ymode=log,
        xlabel= \(\lEsNO\) (dB),
        ylabel= BER,
        xmin=6.4, xmax=6.7,
        ymin = 0.00000000001, ymax = 0.1,
        width=\linewidth,
        height=0.7\linewidth,
        grid=major,
        legend pos=south west,
        legend cell align={left},
        legend style={
            font=\small,
            at={(0,1.05)},anchor=south west
        },
        legend columns=2,
        legend cell align={left},
    ]

    \addlegendimage{very thick, solid, color=black, mark=x, mark options={solid, scale=1}, mark options={solid}}
    \addlegendentry{With Removal}

    \addlegendimage{very thick, solid, color=tab0, mark=x, mark options={solid, scale=1}, mark options={solid}}
    \addlegendentry{20 Iteration}

    \addlegendimage{very thick, dashed, color=black, mark=x, mark options={solid, scale=1}, mark options={solid}}
    \addlegendentry{Without Removal}

    \addlegendimage{very thick, solid, color=tab1, mark=x, mark options={solid, scale=1}, mark options={solid}}
    \addlegendentry{40 Iteration}
    
    \addplot[very thick, tab0, mark=x, mark options={solid, scale=1}] table[col sep=semicolon, skip first n=36, x index=0, y expr={\thisrowno{1} < 1e-12 ? 9e-12: \thisrowno{1}}] {plots/31_07_stall_pattern_removal_of_17_07_ber_curve_ber_sb_1e9_i20_b5_all_params_trial2.txt};

    \addplot[very thick, tab0, dashed, mark=x, mark options={solid, scale=1}] table[col sep=semicolon, skip first n=36, x index=0, y expr={\thisrowno{1} < 1e-12 ? 9e-12: \thisrowno{1}}] {plots/31_07_stall_pattern_removal_off_of_17_07_ber_curve_ber_sb_1e9_i20_b5_all_params_trial2.txt};

    \addplot[very thick, tab1, mark=x, mark options={solid, scale=1}] table[col sep=semicolon, skip first n=36, x index=0, y expr={\thisrowno{1} < 1e-12 ? 9e-12: \thisrowno{1}}] {plots/31_07_stall_pattern_removal_of_17_07_ber_curve_tb_1e-4_i40_b5_11_07_trial1_no_increase_step.txt};

    \addplot[very thick, tab1, dashed, mark=x, mark options={solid, scale=1}] table[col sep=semicolon, skip first n=26, x index=0, y expr={\thisrowno{1} < 1e-12 ? 9e-12: \thisrowno{1}}] {plots/17_07_ber_curve_tb_1e-4_i40_b5_11_07_trial1_no_increase_step.txt};
\end{axis}
\end{tikzpicture}
